Chain of Alignment: Integrating Public Will with Expert Intelligence for Language Model Alignment

We introduce a method to measure the alignment between public will and language model (LM) behavior that can be applied to fine-tuning, online oversight, and pre-release safety checks. Our `chain of alignment' (CoA) approach produces a rule based reward (RBR) by creating model behavior $\textit{rules}$ aligned to normative $\textit{objectives}$ aligned to $\textit{public will}$. This factoring enables a nonexpert public to directly specify their will through the normative objectives, while expert intelligence is used to figure out rules entailing model behavior that best achieves those objectives. We validate our approach by applying it across three different domains of LM prompts related to mental health. We demonstrate a public input process built on collective dialogues and bridging-based ranking that reliably produces normative objectives supported by at least $96\% \pm 2\%$ of the US public. We then show that rules developed by mental health experts to achieve those objectives enable a RBR that evaluates an LM response's alignment with the objectives similarly to human experts (Pearson's $r=0.841$, $AUC=0.964$). By measuring alignment with objectives that have near unanimous public support, these CoA RBRs provide an approximate measure of alignment between LM behavior and public will.

==> util.tex <==
\usepackage{amssymb} % For squares
\usepackage{marginnote} % Lets you have margin things even in figures, minipages, footnotes, etc. in theory. Hacky but used everywhere.
% Alternative https://ctan.org/pkg/minipage-marginpar?lang=en

%%%%%%%%%%%%
% Inline notes
%%%%%%%%%%%%
\newcommand{\note}[1]{ 
    % [{\textcolor{olive}{#1}}]
    % \marginnote{{\textcolor{olive}{note}}}
}

%%%%%%%%%%%%
% Boxes for longer notes
%%%%%%%%%%%%
\usepackage{tcolorbox}
\tcbuselibrary{many}
\usepackage[hybrid]{markdown} 
% Ideally figure out a way to put a \begin{markdown} environment inside this, that would be even better than this weird wiki syntax.

\newenvironment{notes} 
{\begin{tcolorbox}} 
{\end{tcolorbox}}

\newenvironment{meta} 
{\begin{tcolorbox}[colback=red!5!white,colframe=red!75!black]} 
{\end{tcolorbox}}

%%%%%%%%%%%%
% TODO's
%%%%%%%%%%%%
\newcommand\mycheckbox{$\blacksquare $}
\usepackage[colorinlistoftodos]{todonotes}
% Let's you keep a list of TODO's. Also has some very nice in your face TODO's using margin notes, but we might not want that (see detailed comments below). 

% Toggle them on and off, and inclusion into the master todolist by commenting in/out the relevant lines.

% TODOs that are blocking immediate next steps
\newcommand{\todoNow}[1]{ 
    [{\color{red}{#1}\marginnote{do now}}]
    \addcontentsline{tdo}{todo}{{\color{red}{\mycheckbox\mycheckbox}} #1}
}
% TODOs required for the next phase (e.g. publication, broader sharing, etc.)
\newcommand{\todoPhase}[1]{ 
    % [{\color{orange}{#1}\marginnote{phase todo}}]
    % \addcontentsline{tdo}{todo}{{\color{orange}{\mycheckbox}} #1}
}
% EXTERNAL COMMENTS
\newcommand{\feedback}[1]{ 
    % [{\color{olive}{#1}\marginnote{feedback}}]
    % \addcontentsline{tdo}{todo}{{\color{olive}{\mycheckbox}} #1}
}

% Things that should have citations
\newcommand{\todoCite}[1]{ % For 
    % [{\color{teal}{cite \S\ #1}\marginnote{cite}}]
    % \addcontentsline{tdo}{todo}{{\color{teal}{\mycheckbox}} cite \S\ #1}
}
% All other TODOs (e.g. backlog).
\newcommand{\todoLater}[1]{ 
    % [{\color{yellow!60!black}{#1}\marginnote{backlog}}]
    % \addcontentsline{tdo}{todo}{{\color{yellow!60!black}{\mycheckbox}} #1}
}

% Show list of TODO's without ugly links:

% Example outputs for \todo: https://tex.stackexchange.com/a/616037/80414
% Syntax:
%   \todo[color=blue!40]{Todonote with a different color.}
%   \todo[nolist]{Todonote that is only shown in the margin and not in the list of todos.}%
%   \todo[size=\small]{A note with a small fontsize.}
%   \todo[noline]{A note with no line back to the text.}
%   \todo[inline, color=red!50]{Inline todonotes.}
% 
% Example defining different priority levels of TODO:
%   \newcommand{\todoA}[2][]{\todo[color=red!70, inline, #1]{#2}}
%   \newcommand{\todoB}[2][]{\todo[color=orange, inline,#1]{#2}}
%   \newcommand{\todoC}[2][]{\todo[color=yellow!80!black, inline, #1]{#2}}
% 
% Note: "It is not possible to insert todonotes into math environments or floating environments like figure or table. By replacing the marginpar command with a marginnote this can be enabled. For todos inside math environments the todo must be placed in an mbox or \textrm command." e.g.:
% \usepackage{marginnote}
% \let\marginpar\marginnote
% 
% The problem with using todonotes this directly is it's very in your face, and you don't always want that. So instead use inline colored text and use "\addcontentsline{tdo}{todo}{#1}" to add the content of the TODO to the todolist for linking. 


